PartialFormer: Modeling Part Instead of Whole for Machine Translation

The design choices in Transformer feed-forward neural networks have resulted in significant computational and parameter overhead. In this work, we emphasize the importance of hidden dimensions in designing lightweight FFNs, a factor often overlooked in previous architectures. Guided by this principle, we introduce PartialFormer, a parameter-efficient Transformer architecture utilizing multiple smaller FFNs to reduce parameters and computation while maintaining essential hidden dimensions. These smaller FFNs are integrated into a multi-head attention mechanism for effective collaboration. We also propose a tailored head scaling strategy to enhance PartialFormer's capabilities. Furthermore, we present a residual-like attention calculation to improve depth scaling within PartialFormer. Extensive experiments on 9 translation tasks and 1 abstractive summarization task validate the effectiveness of our PartialFormer approach on machine translation and summarization tasks. Our code would be available at: https://github.com/zhengkid/PartialFormer.

==> Figure/Analysis/Hyper-Parameter_Analysis.tex <==
% \definecolor{tiffanyblue}{RGB}{129,216,208}
% \definecolor{bangdiblue}{RGB}{0,149,182}
% \definecolor{kleinblue}{RGB}{0,47,167}
% \definecolor{kabuliblue}{RGB}{26,85,153}
% \definecolor{purple}{RGB}{138,43,226}
% \begin{figure}[ht!]
%     \centering
%   \begin{tikzpicture}[]
%   \pgfplotsset{set layers}
%      \scriptsize{
%       \begin{axis}[
% 	 at={(0,0)},
%       ymajorgrids,
%       xmajorgrids,
%       grid style=dashed,
%       width=0.19\textwidth,
%       height=.25\textwidth,
%       legend style={at={(0.23,0.08)}, anchor=south west},
%       xlabel={\small{\makecell{Encoder Heads \\ (a)}}},
%       ylabel={\small{BLEU}},
%       ylabel style={yshift=-2em},xlabel style={yshift=1.0em},
%       yticklabel style={/pgf/number format/precision=1,/pgf/number format/fixed zerofill},
%       ymin=28.8,ymax=29.7, ytick={28.9, 29.2, 29.5},
%       xmin=14,xmax=32,xtick={16, 24,30},
%       legend style={yshift=-0.5em,xshift=4em,inner sep=1pt,legend plot pos=right,font={\footnotesize},cells={anchor=west}}
%       ]
%       % \draw[|-|,line width=0.6pt, black!80, dashed, thick] (62,31.23) -- (110, 31.23);
%       % using "mark options" do more changes for marks
      
      
%       \addplot[red,mark=otimes*,mark size=2pt,thick,mark options={fill=red,draw=red,line width=1.25pt}] coordinates { 
% (16,28.94)
% (24,29.23)
% (30,29.58)

% % (15,29.33)
% % % (24,29.23)
% % (30,29.58)
      
%       };\label{baseline}
      

      
%       \end{axis}






%     \begin{axis}[
% 	 at={(0.16\textwidth,0)},
%       ymajorgrids,
%       xmajorgrids,
%       grid style=dashed,
%       width=0.19\textwidth,
%       height=.25\textwidth,
%       legend style={at={(0.23,0.08)}, anchor=south west},
%       xlabel={\small{\makecell{Encoder Heads \\ (b)}}},
%       ylabel={\small{$N_{\mathrm{activation}}$}},
%       ylabel style={yshift=-2em},xlabel style={yshift=1.0em},
%       yticklabel style={/pgf/number format/precision=1,/pgf/number format/fixed zerofill},
%       ymin=37,ymax=47, ytick={38, 42, 46},
%       xmin=14,xmax=32,xtick={16, 24,30},
%       legend style={draw=none,yshift=8em,xshift=-11em,inner sep=1pt,legend plot pos=right,font={\small},cells={anchor=west}}
%       ]
%       % \draw[|-|,line width=0.6pt, black!80, dashed, thick] (62,31.23) -- (110, 31.23);
%       % using "mark options" do more changes for marks
      
      
%       \addplot[red,mark=otimes*,mark size=2pt,thick,mark options={fill=red,draw=red,line width=1.25pt}] coordinates { (16, 38.36) (24, 43) (30,46)
%       };

%       % \addplot[blue,line width=2.5pt] coordinates { (16, 35) (30,35)
%       % };
      
      


      
%       \end{axis}


%     \begin{axis}[
% 	 at={(0.32\textwidth,0)},
%       ymajorgrids,
%       xmajorgrids,
%       grid style=dashed,
%       width=0.19\textwidth,
%       height=.25\textwidth,
%       legend style={at={(0.23,0.08)}, anchor=south west},
%       xlabel={\small{\makecell{Encoder Heads \\ (b)}}},
%       ylabel={\small{$\mathrm{Param}_\mathrm{ffn}$~(M)}},
%       ylabel style={yshift=-2em},xlabel style={yshift=1.0em},
%       yticklabel style={/pgf/number format/precision=2,/pgf/number format/fixed zerofill},
%       ymin=0.26,ymax=0.54, ytick={0.3, 0.4, 0.5},
%       xmin=14,xmax=32,xtick={16, 24,30},
%       legend style={draw=none,yshift=9.5em,xshift=-14em,inner sep=1pt,legend plot pos=right,font={\small},cells={anchor=west}}
%       ]
%       % \draw[|-|,line width=0.6pt, black!80, dashed, thick] (62,31.23) -- (110, 31.23);
%       % using "mark options" do more changes for marks
      
      
%       \addplot[red,mark=otimes*,mark size=2pt,thick,mark options={fill=red,draw=red,line width=1.25pt}] coordinates { (16, 0.28) (24, 0.41) (30,0.5022)
%       };
%       \addlegendentry{\scalebox{1}{PartialFormer}}

%       % \addplot[blue,line width=2.5pt] coordinates { (16, 35) (30,35)
%       % };
      
      


      
%       \end{axis}

      
%      }

   
      
      
    



    
      
      
%   \end{tikzpicture}
% \vskip -0.1in
%     \caption{Hyper-Parameter Analysis on the WMT'14 En-De task. }
%     \label{fig:head_vs_bleu_efficiency}
% \end{figure}




\definecolor{tiffanyblue}{RGB}{129,216,208}
\definecolor{bangdiblue}{RGB}{0,149,182}
\definecolor{kleinblue}{RGB}{0,47,167}
\definecolor{kabuliblue}{RGB}{26,85,153}
\definecolor{purple}{RGB}{138,43,226}
\begin{figure}[ht!]
    \centering
  \begin{tikzpicture}[]
  \pgfplotsset{set layers}
     \scriptsize{
      \begin{axis}[
      align=center,
	 at={(0,0)},
      ymajorgrids,
      xmajorgrids,
      grid style=dashed,
      width=0.5\textwidth,
      height=.26\textwidth,
      legend style={at={(0.23,0.08)}, anchor=south west},
      xlabel={\small \makecell{Layer Index
      \\ {(a) }}},
      ylabel={\small{$\eta_{\mathrm{ffn}}$}},
      ylabel style={yshift=-1.5em},xlabel style={yshift=1.0em},
      yticklabel style={/pgf/number format/precision=0,/pgf/number format/fixed zerofill},
      ymin=10,ymax=230, ytick={ 40, 80, 120, 160, 200},
      xmin=0,xmax=25,xtick={1, 6, 12, 18, 24},
      legend style={fill opacity=0.7,draw=none,yshift=4.8em,xshift=-1.1em,inner sep=0pt,legend plot pos=right,font={\small},cells={anchor=west}, legend columns = 1, ,column sep=1pt}
      ]
    
      
      
      \addplot[blue,mark=diamond*,mark size=0.5pt,thick,mark options={fill=blue,draw=blue,line width=1.25pt}] coordinates { (1, 37.49055099487305) (2, 33.633731842041016) (3, 11.66319465637207) (4, 59.70111846923828) (5, 27.588764190673828) (6, 18.19449806213379) (7, 26.111190795898438) (8, 39.12969970703125) (9, 67.24352264404297) (10, 125.52139282226562) (11, 76.20858764648438) (12, 49.84814453125) (13, 61.22653579711914) (14, 46.456993103027344) (15, 114.80828094482422) (16, 47.92739486694336) (17, 56.09264373779297) (18, 12.07628059387207) (19, 24.73710060119629) (20, 39.97461700439453) (21, 30.041296005249023) (22, 40.958988189697266) (23, 31.894935607910156) (24, 27.257652282714844)


      };\label{baseline}
\addlegendentry{\scalebox{0.7}{PartialFormer~($H=23$, $d^h=60$, BLEU: 29.23)}}



       
     
      

    


     
 
      \addplot[red, mark=otimes*,mark size=0.5pt,thick,mark options={fill=red,draw=red,line width=1.25pt}] coordinates { (1, 58.622589111328125) (2, 69.19847869873047) (3, 27.586591720581055) (4, 60.08373260498047) (5, 202.59915161132812) (6, 38.71195983886719) (7, 8.798989295959473) (8, 99.24288940429688) (9, 65.37349700927734) (10, 31.127098083496094) (11, 80.68778228759766) (12, 93.42373657226562) (13, 177.79580688476562) (14, 149.07830810546875) (15, 115.77934265136719) (16, 107.13433837890625) (17, 117.249267578125) (18, 102.11153411865234) (19, 110.17288970947266) (20, 85.04967498779297) (21, 115.41409301757812) (22, 77.47010803222656) (23, 132.24522399902344) (24, 82.13630676269531)

      };
      \addlegendentry{\scalebox{0.7}{PartialFormer~($H=30$, $d^h=45$, BLEU: 29.58)}}

\addplot[blue!30, line width=2.5pt] coordinates { (1, 46.0745) (24, 46.0745)
      };
      
        \addplot[red!30,line width=2.5pt] coordinates { (1, 91.9622)  (24, 91.9622)

      };

%     \draw[<-, thick] (axis cs:13, 91.9622) -- (axis cs:13,35.7504) ;
% % \draw[->, thick] (axis cs:0, 0) -- (axis cs:5.5, 12.65) ;
% \node[anchor=west,font=\footnotesize] at (axis cs:13, 63.8563) {\bf 2.6$\mathbf{\times\uparrow}$ };
      
      
      \end{axis}






     }

   
    
  


    
      
      
  \end{tikzpicture}
\vskip -0.1in
    \caption{Comparison of the efficiency of FFN (higher is better) in Transformer and PartialFormer.  }
    \label{fig:more_analysis}
\end{figure}

==> Figure/Analysis/More_Analysis.tex <==
\definecolor{tiffanyblue}{RGB}{129,216,208}
\definecolor{bangdiblue}{RGB}{0,149,182}
\definecolor{kleinblue}{RGB}{0,47,167}
\definecolor{kabuliblue}{RGB}{26,85,153}
\definecolor{purple}{RGB}{138,43,226}
\begin{figure*}[ht!]
    \centering
  \begin{tikzpicture}[]
  \pgfplotsset{set layers}
     \scriptsize{
      \begin{axis}[
      align=center,
	 at={(0,0)},
      ymajorgrids,
      xmajorgrids,
      grid style=dashed,
      width=0.33\textwidth,
      height=.22\textwidth,
      legend style={at={(0.23,0.08)}, anchor=south west},
      xlabel={\small \makecell{Layer Index
      \\ {(a) }}},
      ylabel={\small{$\eta_{\mathrm{ffn}}$}},
      ylabel style={yshift=-1.5em},xlabel style={yshift=1.0em},
      yticklabel style={/pgf/number format/precision=0,/pgf/number format/fixed zerofill},
      ymin=20,ymax=220, ytick={ 40, 80, 120, 160, 200},
      xmin=0,xmax=25,xtick={1, 6, 12, 18, 24},
      legend style={draw=none,yshift=8em,xshift=6em,inner sep=0pt,legend plot pos=right,font={\small},cells={anchor=west}, legend columns = 2, ,column sep=5pt}
      ]
    
      
      
      \addplot[blue,mark=diamond*,mark size=0.5pt,thick,mark options={fill=blue,draw=blue,line width=1.25pt}] coordinates { (1, 50.397850036621094) (2, 46.05617141723633) (3, 30.716957092285156) (4, 32.27601623535156) (5, 28.592182159423828) (6, 25.675628662109375) (7, 24.729618072509766) (8, 28.869112014770508) (9, 26.933958053588867) (10, 30.077404022216797) (11, 33.576473236083984) (12, 31.970033645629883) (13, 32.3390998840332) (14, 33.447723388671875) (15, 33.69960021972656) (16, 31.835311889648438) (17, 31.542987823486328) (18, 34.97138595581055) (19, 35.815101623535156) (20, 36.96128845214844) (21, 40.59370803833008) (22, 43.48105239868164) (23, 50.58210754394531) (24, 62.86782455444336)


      };\label{baseline}
\addlegendentry{\scalebox{1}{Transformer~(BLEU: 28.00)}}


       
     
      

    


     
 
      \addplot[red, mark=otimes*,mark size=0.5pt,thick,mark options={fill=red,draw=red,line width=1.25pt}] coordinates { (1, 58.622589111328125) (2, 69.19847869873047) (3, 27.586591720581055) (4, 60.08373260498047) (5, 202.59915161132812) (6, 38.71195983886719) (7, 8.798989295959473) (8, 99.24288940429688) (9, 65.37349700927734) (10, 31.127098083496094) (11, 80.68778228759766) (12, 93.42373657226562) (13, 177.79580688476562) (14, 149.07830810546875) (15, 115.77934265136719) (16, 107.13433837890625) (17, 117.249267578125) (18, 102.11153411865234) (19, 110.17288970947266) (20, 85.04967498779297) (21, 115.41409301757812) (22, 77.47010803222656) (23, 132.24522399902344) (24, 82.13630676269531)

      };
      \addlegendentry{\scalebox{1}{PartialFormer~(BLEU: 29.58)}}

\addplot[blue!30, line width=2.5pt] coordinates { (1, 35.7504) (24, 35.7504)
      };
      
        \addplot[red!30,line width=2.5pt] coordinates { (1, 91.9622)  (24, 91.9622)

      };

    \draw[<-, thick] (axis cs:13, 91.9622) -- (axis cs:13,35.7504) ;
% \draw[->, thick] (axis cs:0, 0) -- (axis cs:5.5, 12.65) ;
\node[anchor=west,font=\footnotesize] at (axis cs:13, 63.8563) {\bf 2.6$\mathbf{\times\uparrow}$ };
      
      
      \end{axis}





    \begin{axis}[
	 at={(0.33\textwidth,0)},
      ymajorgrids,
      xmajorgrids,
      grid style=dashed,
      width=0.33\textwidth,
      height=.22\textwidth,
      legend style={at={(0.23,0.08)}, anchor=south west},
      xlabel={\small \makecell{Layer Index
      \\ {(b) }}},
      ylabel={\small{Head Diversity}},
      ylabel style={yshift=-1.5em},xlabel style={yshift=1.0em},
      yticklabel style={/pgf/number format/precision=2,/pgf/number format/fixed zerofill},
      ymin=0.76,ymax=0.94, ytick={ 0.79, 0.82, 0.85, 0.88, 0.91},
      xmin=0,xmax=25,xtick={1, 6, 12, 18, 24},
      legend style={yshift=-0.5em,xshift=4em,inner sep=1pt,legend plot pos=right,font={\small},cells={anchor=west}}
      ]
      % \draw[|-|,line width=0.6pt, black!80, dashed, thick] (62,31.23) -- (110, 31.23);
      % using "mark options" do more changes for marks
      
      
      \addplot[blue,mark=diamond*,mark size=0.5pt,thick,mark options={fill=blue,draw=blue,line width=1.25pt}] coordinates { (1,0.7942273020744324)
(2,0.7962304353713989)
(3,0.7946145534515381)
(4,0.7945131659507751)
(5,0.7952606081962585)
(6,0.7940300703048706)
(7,0.7944667339324951)
(8,0.7958396077156067)
(9,0.7942259907722473)
(10,0.7952779531478882)
(11,0.7945087552070618)
(12,0.795943558216095)
(13,0.7943979501724243)
(14,0.7950928211212158)
(15,0.7946134805679321)
(16,0.7939436435699463)
(17,0.7947837114334106)
(18,0.7948220372200012)
(19,0.7949259281158447)
(20,0.7952647805213928)
(21,0.7957655787467957)
(22,0.7956266403198242)
(23,0.7946876287460327)
(24,0.7941218018531799)


      };
     
      

  
      
  \addplot[blue!30,line width=2.5pt] coordinates { (1,0.7949)
(24,0.7949)
      };

     
 
      \addplot[red, mark=otimes*,mark size=0.5pt,thick,mark options={fill=red,draw=red,line width=1.25pt}] coordinates { (1,0.9289955496788025)
(2,0.9303833246231079)
(3,0.9280907511711121)
(4,0.9178294539451599)
(5,0.9058080315589905)
(6,0.9134395718574524)
(7,0.9192654490470886)
(8,0.9071937799453735)
(9,0.9131340980529785)
(10,0.9085556268692017)
(11,0.9041228890419006)
(12,0.9006943106651306)
(13,0.906696081161499)
(14,0.9062924385070801)
(15,0.902535617351532)
(16,0.9111884832382202)
(17,0.9071165323257446)
(18,0.8982360363006592)
(19,0.9003955721855164)
(20,0.8912466764450073)
(21,0.8940209746360779)
(22,0.8901423811912537)
(23,0.894454300403595)
(24,0.8898761868476868)


      };

       \addplot[red!30, line width=2.5pt] coordinates { (1,0.9071)
(24,0.9071)
      };

      \draw[<-, thick] (axis cs:7, 0.9071) -- (axis cs:7,0.7949) ;
% \draw[->, thick] (axis cs:0, 0) -- (axis cs:5.5, 12.65) ;
\node[anchor=west,font=\footnotesize] at (axis cs:7, 0.8510) {\bf 1.1$\mathbf{\times \uparrow} $ };

      \end{axis}

    \begin{axis}[
	 at={(0.66\textwidth,0)},
      ymajorgrids,
      xmajorgrids,
      grid style=dashed,
      width=0.33\textwidth,
      height=.22\textwidth,
      legend style={at={(0.23,0.08)}, anchor=south west},
      xlabel={\small \makecell{Layer Index
      \\ {(c) }}},
      ylabel={\small{Smoothing Rate}},
      ylabel style={yshift=-1.5em},xlabel style={yshift=1.0em},
      yticklabel style={/pgf/number format/precision=2,/pgf/number format/fixed zerofill},
      ymin=0,ymax=0.6, ytick={ 0.1, 0.2, 0.3, 0.4, 0.5},
      xmin=0,xmax=25,xtick={1, 6, 12, 18, 24},
      legend style={yshift=-0.5em,xshift=4em,inner sep=1pt,legend plot pos=right,font={\footnotesize},cells={anchor=west}}
      ]
      % \draw[|-|,line width=0.6pt, black!80, dashed, thick] (62,31.23) -- (110, 31.23);
      % using "mark options" do more changes for marks
      
      
      \addplot[blue,mark=diamond*,mark size=0.5pt,thick,mark options={fill=blue,draw=blue,line width=1.25pt}] coordinates { (1, 0.28883352875709534) (2, 0.41732001304626465) (3, 0.4699432849884033) (4, 0.4995066225528717) (5, 0.5271627306938171) (6, 0.5504211783409119) (7, 0.5659817457199097) (8, 0.5709900259971619) (9, 0.5731505751609802) (10, 0.570284366607666) (11, 0.5726948976516724) (12, 0.5708319544792175) (13, 0.563860297203064) (14, 0.5604643225669861) (15, 0.5560687780380249) (16, 0.5486728549003601) (17, 0.5399861335754395) (18, 0.5283432602882385) (19, 0.5198920965194702) (20, 0.5089938640594482) (21, 0.498872846364975) (22, 0.49158498644828796) (23, 0.48306941986083984) (24, 0.47021931409835815)

      };
      % \addlegendentry{\scalebox{.6}{Transformer}}


      \addplot[blue!30,line width=2.5pt] coordinates { (1, 0.5186) (24, 0.5186)

      };

    


     
 
      \addplot[red, mark=otimes*,mark size=0.5pt,thick,mark options={fill=red,draw=red,line width=1.25pt}] coordinates { (1, 0.05046646296977997) (2, 0.06599926948547363) (3, 0.08231858164072037) (4, 0.10168235003948212) (5, 0.11680775880813599) (6, 0.1316044181585312) (7, 0.14767728745937347) (8, 0.16397510468959808) (9, 0.17946700751781464) (10, 0.19437670707702637) (11, 0.2057010680437088) (12, 0.21689032018184662) (13, 0.2251075953245163) (14, 0.23383928835391998) (15, 0.2391471564769745) (16, 0.24002841114997864) (17, 0.24297945201396942) (18, 0.24586531519889832) (19, 0.2480057328939438) (20, 0.2517806589603424) (21, 0.2551610767841339) (22, 0.2591455578804016) (23, 0.26618409156799316) (24, 0.2723335921764374)

      };
      

      \addplot[red!30, line width=2.5pt] coordinates { (1, 0.1932)  (24, 0.1932)

     

      };

      \draw[<-, thick] (axis cs:7, 0.1932) -- (axis cs:7,0.5186) ;
% \draw[->, thick] (axis cs:0, 0) -- (axis cs:5.5, 12.65) ;
\node[anchor=west,font=\footnotesize] at (axis cs:7, 0.3559) {\bf 2.7$\mathbf{\times \downarrow}$ };

      
      \end{axis}
      
     }

   
    
  


    
      
      
  \end{tikzpicture}
\vskip -0.1in
    \caption{(a) Comparison of the efficiency of FFN (higher is better) in Transformer and PartialFormer. (b) Comparison of Head diversity (higher is better) in Transformer and PartialFormer. Following \cite{li-etal-2018-multi-head}, we measure the diversity of head representation via negative cosine similarity. (3) Comparison of smoothing rate diversity (lower is better) in Transformer and PartialFormer. }
    \label{fig:more_analysis}
\end{figure*}
